WorldSculpt: Generating Compositional Worlds from Grounded Videos

We study the problem of generating a compositional 3D representation of a cluttered scene containing hundreds of objects. The goal is to represent the scene as a collection of individual object meshes placed in a shared world frame, as required by downstream applications such as gaming, AR/VR, simulation, and robotics. This task is challenging in densely cluttered scenes, where objects heavily occlude one another and each view reveals only a fraction of their geometry. Geometry-based approaches typically reconstruct the scene as a single representation and leave incomplete geometry in occluded regions, while existing compositional methods with generative priors are largely limited to relatively simple scenes. We show that complex scenes with hundreds of objects can instead be generated compositionally by adapting a strong single-object 3D generative prior to multi-view observations. We instantiate this paradigm with Pixal3D, extending it with a multi-view conditioning pathway that grounds object generation in multiple posed observations. Although the model is finetuned entirely on single objects in canonical space, it generalizes to large scenes with severe occlusion without any scene-level training, demonstrating the feasibility and scalability of this paradigm. We further introduce UE-MeshyScene, a photorealistic benchmark of densely cluttered scenes with hundreds of objects, per-object annotations, and ground-truth meshes. Across single-object, controlled multi-object, and UE-MeshyScene evaluations, our method consistently outperforms prior approaches, with larger gains as scene complexity and occlusion increase. Finally, we demonstrate broader applicability by converting generated 3DGS worlds, such as Marble and HY-World 2.0, into compositional mesh scenes.

==> sec/FLUIDdata.tex <==
\section{FLUID Dataset}

The novelty of our \textbf{FLUID dataset} lies in two major aspects:

\begin{enumerate}
    \item \textbf{Closer to realistic interactive scenarios.} 
    Unlike existing datasets (e.g., Meta’s dataset) that mostly simulate two participants engaged in remote, disjoint conversations without physical embodiment, FLUID captures richer and more natural human interactions. In particular, it incorporates \textbf{action-based interactions} and \textbf{action interruptions}, which are critical for modeling dynamic and fluid exchanges in real-world communication.
    
    \item \textbf{Support for multimodal close interaction and 3D reconstruction.}
    Current datasets lack the ability to support 3D reconstruction and do not include physical interactions such as gestures, expressions, or proximity-based behaviors. FLUID is designed as an \textbf{extended version of Harmony4D}, enriched with \textbf{dialogue and close-proximity interactions} between participants. This extension is essential for training AI systems capable of learning \textbf{action- and expression-driven interaction} beyond mere speech exchange.
\end{enumerate}

By introducing these innovations, FLUID provides a unique benchmark for advancing digital humans toward more \textbf{embodied, multimodal, and contextually grounded interaction intelligence}.

